Linguistic Versus Latent Relations for Modeling Coherent Flow in Paragraphs

Generating a long, coherent text such as a paragraph requires a high-level control of different levels of relations between sentences (e.g., tense, coreference). We call such a logical connection between sentences as a (paragraph) flow. In order to produce a coherent flow of text, we explore two forms of intersentential relations in a paragraph: one is a human-created linguistical relation that forms a structure (e.g., discourse tree) and the other is a relation from latent representation learned from the sentences themselves. Our two proposed models incorporate each form of relations into document-level language models: the former is a supervised model that jointly learns a language model as well as discourse relation prediction, and the latter is an unsupervised model that is hierarchically conditioned by a recurrent neural network (RNN) over the latent information. Our proposed models with both forms of relations outperform the baselines in partially conditioned paragraph generation task. Our codes and data are publicly available.

==> 02analysis.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Linguistic vs Latent Relations}\label{sec:motivation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\hh{change ``type'' to ``form''.}\dk{Changed.}

We describe two forms of inter-sentential 
% \hh{not both are inter-sentential, as we discussed.}\dk{I added a foonote for clarification. What do you think?} 
relations\footnote{The segment of sentence could be either an individual sentence or a phrase parsed by a discourse parser called an elementary discourse units (EDU).} in a paragraph: discourse and delta relations.
% We first provide a preliminary observation and motivation behind why we choose them, and summarize their fundamental difference in nature.
% first discuss the importance of the form by showing observations on preliminary experiments. 

Discourse analysis studies how a document is composed at different dimensions such as gestures, syntax, lexicon, style, rhetoric, meanings, strategies, and other aspects of interaction. 
Rhetorical Structure Theory (RST)~\cite{mann1988rhetorical} is a discourse analysis theory, which analyzes how we ensure a coherence of a document. 
% It analyzes a document into a tree of nested discourse units.
Parsing a document into a RST tree produces the structural and linguistic relations between sentences and groups of sentences \cite{soricut2003sentence}.

In our modeling, we limit usage of the discourse tree to only relations between adjacent phrases: relations are inserted between adjacent phrases and represented as a flattened sequence of phrases and relations \footnote{If we meet two consecutive RST relations, we accept the deeper level of relation to preserve detailed relation. In case that the central EDU is after its dependent where the EDUs may not be semantically related in the flattened sequence, we don't include the relation.}.

Each sequence of the flattened discourse relations may correspond to a generic writing flow.
% \tj{What is the previous word 'la'? I couldn't change it since I don't know what it means.}
%\hh{until here, I don't think we need to mention.}
% \hh{For this, I would put like: According to RST, a common way of relating two units is ``Elaboration'', blah blah.}\dk{Why do we need to say the most frequent relation type intead of two sequence of two types?}
For example, people often write a text by elaborating basic information (\texttt{Elaboration}) and then describing a following statement attributed to the information (\texttt{Attribution}).
If we extend it to a full sequence of RST relations in a paragraph and incorporate them into text generation, we may model a partial\footnote{Since we flatten the discourse tree, we lose the information from the tree hierarchy.} high-level flow of text conditioned by the RST relations. 
% We propose a discourse-relat

Another form we discuss is a latent representation called \textit{delta} learned %\hh{Not could be. You learn them right.}\dk{Fixed}
from adjacent sentences directly.
Most modern prior work focuses on modeling inter-sententional relation by hierarchically modeling sequences of words and sentences at the same time~\cite{lin2015hierarchical,chung2016hierarchical}.
% However, sequence of sentences in the hierarchical model is specific to topics of the given document instead of writing flows which is independent to the topic.
However, a sequence of sentences in the hierarchical models is limited to modeling topic transitions between sentences, while our aim is to characterize high-level flow (i.e., writing schemes), which is independent of the topic.
%\hh{I don't understand this sentence.}\dk{How about now?} 
%For example, a general flow could be either applied to a document about either sports or politics.  %\hh{``plan'' used.}\dk{removed.}

Before empirical comparison of the two forms of relations, we summarize the fundamental differences of the two forms as follows:
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
\item While labels in linguistic relations are interpretable, accuracy of the labels highly depends on the performance of the discourse parser. On the other hand, latent representations with delta operation do not suffer from out-of-domain or accuracy problems that external parsers may bring in. 
\item Linguistic relations can hold over long distances with many things in between (e.g., Solutionhood), while the latent ones are always immediately adjacent.  
\item Linguistic ones are fairly coarse-grained and non-continuous, often making them inapplicable to other continuous models (e.g., a neural network), while latent ones are by definition continuous, always making them applicable.
\item Linguistic relations are often ambiguous or unclear, while latent ones can easily hybridize and represent two more relations at the same time, at the cost of being indefinable.  
\end{itemize}



% %%%%%%%%%%%%%%%%%%%%
% \subsection{Discourse Relations}\label{sec:discourse}
% %%%%%%%%%%%%%%%%%%%%
% %\hh{RST is a theory about how we compose a document. }\dk{Added. See below.}
% % \cite{fox1993discourse}
% Discourse analysis studies how a document is composed at different dimensions such as gestures, syntax, lexicon, style, rhetoric, meanings, strategies, and other aspects of interaction. 
% Rhetorical Structure Theory (RST)~\cite{mann1988rhetorical} is a discourse analysis theory, which analyzes how we ensure a coherence of a document. 
% It analyzes a document into a tree of nested discourse units.
% Parsing a document into a RST tree produces the structural and linguistic relations between sentences and groups of sentences \cite{soricut2003sentence}.

% % (SEQUENCE (CONSEQUENCE e1 e2) (CIRCUMSTANCE e3 e4))
% \begin{figure}[ht]
% \vspace{-3mm}
% \tiny
% {\hspace{0pt}\setlength{\linewidth}{60pt}
% \dirrel{SEQUENCE}{
%   \dirrel{CONSEQUENCE}{\rstsegment{\refr{bush1}}}
%   {}{\rstsegment{\refr{bush2}}}
% }
% {}{
%   \dirrel{CIRCUMSTANCE}{\rstsegment{\refr{bush3}}}
%   {}{\rstsegment{\refr{bush4}}}
% }\vspace{0mm}
% \begin{rhetoricaltext}
% \small
% \unit[bush1]{On Aug. 11, the state tore up its controls,} \textcolor{red}{CONSEQUENCE}
% \unit[bush2]{and food prices leaped}\textcolor{red}{SEQUENCE}
% \unit[bush3]{Without buffer stocks,}\textcolor{red}{CIRCUMSTANCE}
% \unit[bush4]{inflation exploded.}
% %\source{wsj$_{2326}$}
% \end{rhetoricaltext}
% }\vspace{-4mm}
% \caption{A parsed RST discourse tree (top) and its flattened sequence (bottom).} \label{fig:rst_example}
% \vspace{-4mm}
% \end{figure}
% % [On Aug. 11, the state tore up its controls,]$_{e1}$ [and food prices leaped]$_{e2}$ [Without buffer stocks,]$_{e3}$ [inflation exploded.]$_{e4}$.



% Figure~\ref{fig:rst_example} shows an example parse tree produced by the state-of-the-art discourse parser \cite{ji2014representation} trained on the RST Discourse Treebank~\cite{miltsakaki2004penn}.
% The two sentences are firstly parsed into four elementary discourse units (EDU) %\hh{WTF is EDU? Need description.}\dk{Changed EDU to phrases. I won't use the term EDU anymore.}
% (e.g., 1A), and then relations among them (e.g., SEQUENCE) are predicted.
% Since we limit usage of the discourse tree to only relations between adjacent phrases, the recursive structure needs to be flattened: relations are inserted between adjacent phrases and represented as a flattened sequence of phrases and relations \footnote{If we meet two consecutive RST relations, we accept the deeper level of relation to preserve detailed relation. In case that the central EDU is after its dependent where the EDUs may not be semantically related in the flattened sequence, we don't include the relation.}.


% % \hh{Actually, do we even need the statistics in text form? This can just go to appendices IMO.}\dk{You don't get high level motivation why RST (even sequence of them) relation are useful for better modeling the text sequence? Hmm. I don't know what to do then. } \hh{11/17: IMO, ``NS''-elaboration or ``text.orga'' or such raw relations lead to confusion. I think showing 1) relevant\&frequent relations 2) say that there are patterns of relations, are enough. }
% We parse paragraphs in news %\hh{Wait, is this ``News'' a unique name of the corpus?}\dk{Changed to news articles}
% articles to find the most frequent RST relations. 
% % In this corpus, there are a total of 45 unique RST relations.
% %\footnote{E.g., Antithesis, Background, Circumstance, Concession, Enablement, Evaluation, Evidence, Interpretation, Justify, Motivation, Otherwise, Purpose, Restatement, Summary, Volitional Cause}
% \texttt{Elaboration} is the most frequent relation followed by \texttt{List} and \texttt{Attribution}.
% We also find the two most frequent patterns of two adjacent relations from three phrases: \texttt{Elaboration} $\rightarrow$ \texttt{Attribution} and \texttt{List} $\rightarrow$ \texttt{Attribution}.


% Each sequence of the flattened discourse relations may correspond to a generic writing flow.
% % \tj{What is the previous word 'la'? I couldn't change it since I don't know what it means.}
% %\hh{until here, I don't think we need to mention.}
% % \hh{For this, I would put like: According to RST, a common way of relating two units is ``Elaboration'', blah blah.}\dk{Why do we need to say the most frequent relation type intead of two sequence of two types?}
% For example, people often write a text by elaborating basic information (\texttt{Elaboration}) and then describing a following statement attributed to the information (\texttt{Attribution}).
% If we extend it to a full sequence of RST relations in a paragraph and incorporate them into text generation, we may model a partial\footnote{Since we flatten the discourse tree, we lose the information from the tree hierarchy.} high-level flow of text conditioned by the RST relations. 
% % We propose a discourse-relation conditioned language model in Section \ref{sec:lmdiscourse}. 
% % \hh{Up to this point, I still don't buy why RST should be used to model flat / sequential relations among sentences. I understand, I am picky, but RST is defined over trees.}\dk{I see. Well, I thought that showing some frequent patterns of two length of RST relations would be helpful for understanding that there are frequent patterns used by people in news articles. Any suggestion then? }

% % \dk{Make clear: sentence vs clauses/phrases}



% %%%%%%%%%%%%%%%%%%%%
% \subsection{Delta Relations}\label{sec:implicit}
% %%%%%%%%%%%%%%%%%%%%
% Another form we discuss is a latent representation called \textit{delta} learned %\hh{Not could be. You learn them right.}\dk{Fixed}
% from adjacent sentences directly.
% Most modern prior work focuses on modeling inter-sententional relation by hierarchically modeling sequences of words and sentences at the same time~\cite{lin2015hierarchical,chung2016hierarchical}.
% % However, sequence of sentences in the hierarchical model is specific to topics of the given document instead of writing flows which is independent to the topic.
% However, a sequence of sentences in the hierarchical models is limited to modeling topic transitions between sentences, while our aim is to characterize high-level flow (i.e., writing schemes), which is independent of the topic.
% %\hh{I don't understand this sentence.}\dk{How about now?} 
% %For example, a general flow could be either applied to a document about either sports or politics.  %\hh{``plan'' used.}\dk{removed.}

% \begin{figure}[ht]
% \vspace{0mm}
% \centering\vspace{-3mm}
% % \subfloat[\small{Paragraphs in news articles}]{\includegraphics[trim={11mm 6mm 12mm 5mm},clip,width=0.5\linewidth,height=2.1cm]{figs_delta_new/{nyt_7_all}.png}}
% % \subfloat[\small{Paragraphs in novel books}]{\includegraphics[trim={11mm 6mm 12mm 5mm},clip,width=0.5\linewidth,height=2.1cm]{figs_delta_new/{book_Fantasy_7_all}.png}}\@
% % \vspace{-3mm}\\
% \subfloat[\small{Paragraphs of Introduction sections}]{\includegraphics[trim={11mm 6mm 12mm 5mm},clip,width=0.7\linewidth,height=3.1cm]{figs_delta_new/{topic_arxiv_7_introduction_43}.png}}\vspace{-3mm}\\
% \subfloat[\small{Paragraphs of Result sections}]{\includegraphics[trim={11mm 6mm 12mm 5mm},clip,width=0.7\linewidth,height=3.1cm]{figs_delta_new/{topic_arxiv_7_result_8}.png}}\@ \vspace{-3mm}
% \caption{
% Delta analysis on paragraphs in academic papers. X-axis is $i$th sentence pair in a paragraph, and y-axis is the averaged Euclidean distance (delta) between them with an error bar.
% The larger distance in y-axis, the more meaning difference between sentences.
% There are three types of sentence pairs: {\color{black}{\textbf{black}}} graph is a pair between two adjacent sentences, and {\color{red}{red}} (or {\color{blue}{blue}}) graphs are pairs between the first (or last) sentence and others. Best viewed in color.
% \vspace{-5mm}
% %\hh{Caption is hard to understand.}\dk{How about now?}
% % \tj{Can you change a color or a style(dash?) of the error bar?}
% }  \label{fig:delta_ex}
% \end{figure}




% We first conduct a delta analysis in Figure~\ref{fig:delta_ex}.
% We calculate Euclidean distances 
% %\tj{In figure 3, y-axis is the averaged cosine similarity distance. But you mention here $d(s_{i}, s_{j})$ is a Euclidean distance. Which one is correct?} 
% between pairs of sentence vectors $d (s_i, s_j)= \lVert s_i - s_j \rVert$ from different sections of academic papers; (a) Introduction and (b) Result.
% %\hh{Visual explanation should resolve intricate explanations.}\dk{check that out again.}
% The pair of sentences are chosen between two adjacent sentences; $d(s_i,s_{i+1})$ or between the first (or last) sentence with others; $d(s_{1},s_i)$ (or $d(s_{l},s_i)$) where $l$ is the index of last sentence.
% Each sentence $s_t$ is represented by averaging word vectors from GloVe~\cite{pennington2014glove} in the sentence. %$s_t = \frac{1}{T} \sum_i w_{ti}$.
% % In Figure \ref{fig:delta_ex}, we show the results of the analysis applied to different domains; 


% We observe paragraphs from different domains and from different sections of academic papers have their own delta flows. 
% %We observe different delta flows between news articles (a) and fantasy books (b). 
% % For example, \texttt{News} shows strong dissimilarity between the first and the last sentence, which indicates that last sentence of News articles are mostly .
% % Paragraphs in Result sections of academic \text{Papers} seem to have
% % We propose a delta-relation conditioned language model in Section \ref{sec:lmdelta}.
% % This is mainly because paragraphs in Introduction often include more general and descriptive text than related work.
% % For example, the distances between the first (or last) and other sentences in novel books (b) gradually rise (or fall), while ones in news articles (a) fluctuate. 
% %, indicating narrative storytelling of paragraphs in novel books. 
% % Most of genres in \texttt{Books} shows gradual rise of deltas ($\Delta_{FA}$) with the first sentence except the last sentence, which means that the first and last sentence are likely similar compared to other corpus. 
% %More delta analysis with different lengths, genres, and topics are in the Appendix for further analysis.
% % \dk{
% % For instance the fact that paragraphs in book evolve less rapidly than News and Sc Papers is certainly mostly due to the fact that books have much more space to communicate information while News must deliver a message with far less space}
% % Not only the different domain, but also the different paragraphs from an academic paper have such different patterns. 
% %Paragraphs in different sections in academic papers also have different information variance between sentences on average. 
% %We suspect this is mainly because people have different strategies or habits of writing sentences according to each section of academic paper or even domain~\footnote{Please find more analysis on paragraphs in different domains such as News and novel books in the Appendix}.
% The distances between adjacent sentences in Introduction sections (a) seem to be more gradual, while those in Result sections (b) are much more fluctuating. It is presumably because text in Result sections tends to be more variable.
% % \tj{there was a wrong analysis for the previous part. I changed 'less' variant --> 'more' variant, and 'similar' meaning --> 'diverse' meaning}
% % We can also observe that the error bar size is wider in the introduction than in the results, which suggests that the writing style
% % of the introduction among different papers varies much more than how people write results.
% These observations motivates that inter-sentential differences (or deltas) may be useful features for modeling the topic-invariant flow of text. 

% \subsection{Theoretical Comparison}
% Before empirical comparison of the two forms of relations, we summarize the fundamental differences of the two forms as follows:
% \begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
% \item While labels in linguistic relations are interpretable, accuracy of the labels highly depends on the performance of the discourse parser. On the other hand, latent representations with delta operation do not suffer from out-of-domain or accuracy problems that external parsers may bring in. 
% \item Linguistic relations can hold over long distances with many things in between (e.g., Solutionhood), while the latent ones are always immediately adjacent.  
% % \tj{please try to change following bullet point. Can't capture the point! For example, what is the feature only linguistic relations can capture?}
% % \item Linguistic relations are defined with explicit labels that latent ones may not be able to represent, while latent ones probably capture some features (e.g.,  tense, topic shift) that linguistic ones never included.  
% \item Linguistic ones are fairly coarse-grained and non-continuous, often making them inapplicable to other continuous models (e.g., a neural network), while latent ones are by definition continuous, always making them applicable.
% \item Linguistic relations are often ambiguous or unclear, while latent ones can easily hybridize and represent two more relations at the same time, at the cost of being indefinable.  
% \end{itemize}
% % Our work studies how these relations learn textual flow, and compares them to conditional text generation tasks.
% %to provide pros and cons of each model.

% % Given the observation from linguistic and latent form of a flow information, 
% % We observe that multiple sentences in a paragraph are written by implicit writing habits such as the first and last sentences should be similar in academic writing or high-level plans of what to say.
% % Those writing habits and plans are difficult to be captured with a simple model.
% % \hh{Orthogonal. Also, we can't say anything about habits or semantic similarity of contents just by looking at annotated discourse relations.}




